ALF: Autoencoder-based Low-rank Filter-sharing for Efficient Convolutional Neural Networks

Closing the gap between the hardware requirements of state-of-the-art convolutional neural networks and the limited resources constraining embedded applications is the next big challenge in deep learning research. The computational complexity and memory footprint of such neural networks are typically daunting for deployment in resource constrained environments. Model compression techniques, such as pruning, are emphasized among other optimization methods for solving this problem. Most existing techniques require domain expertise or result in irregular sparse representations, which increase the burden of deploying deep learning applications on embedded hardware accelerators. In this paper, we propose the autoencoder-based low-rank filter-sharing technique technique (ALF). When applied to various networks, ALF is compared to state-of-the-art pruning methods, demonstrating its efficient compression capabilities on theoretical metrics as well as on an accurate, deterministic hardware-model. In our experiments, ALF showed a reduction of 70\% in network parameters, 61\% in operations and 41\% in execution time, with minimal loss in accuracy.

==> data/30_hwmodel.tex <==
\iffalse
Introduce Memory Hierarchy of Eyeriss (or Eyeriss-like architectures)
\begin{itemize}
    \item Impact of DRAM to SRAM movement ($200\times$ cost of RF read)
    \item Impact of CNN Model size on tiling factors and SRAM capacity
    \item Impact of compressed parameters in reducing computation latency
\end{itemize}

\textit{Briefly} introduce concept of loop blocking/tiling, reordering, unrolling.

\textit{State the deterministic execution of CNNs as a motivation for modelling.} Mention estimation accuracy of model vs. real hw-metrics. Differentiate from NetAdapt naive modelling scheme.
\fi

The deterministic execution of a particular CNN on a target hardware platform eases the creation of hardware models with highly accurate estimates. For the purpose of demonstrating the hardware execution advantages of ALF blocks, we use such a modeling framework, which accurately replicates the execution and scheduling scheme of the Eyeriss accelerator \ref{Eyeriss}.

The energy contribution of data movement cannot be disregarded for efficient execution of CNNs. If left unoptimized, it can easily exceed the energy required by the multitude of computations typical in state-of-the-art neural networks. The Eyeriss architecture is a parallel computation array with 3 levels of memory hierarchy, namely Off-Chip (DRAM), On-Chip (SRAM) and PE Registers. For data movement modeling, transfers between PEs on the Network-on-Chip are modeled as a further memory hierarchy.

CNNs are commonly represented in a nested for-loop format. These for-loops present many reuse opportunities, as the main computation is at the core of the inner-most loop. Due to memory constraints, the parameters required by the entire nested-loop do not fit in the lowest-level of the memory hierarchy. A standard method of exploiting the entire memory hierarchy is to relax this constraint and split the for-loops into shallower loops through a technique called \textiit{loop-blocking}. Once the memory level is distributed spatially, we can unroll the loop over the parallelism degree offered by the hardware architecture through \textiit{loop-unrolling}. We study the extent of these strategies for vanilla state-of-the-art CNNs and their ALF-block variants.

The modeling framework's accuracy is verified against the real hardware results published in \ref{Eyeriss}, as shown in Fig. \ref{fig:}. Furthermore, we restrict the modeling framework from manipulating the loop reordering scheme or mapping cost function, such that the differences observed in any experiments purely depend on the structure of the executed CNN.

==> data/alf_algo.tex <==
For a clear overview, Algorithm~\ref{alg:ae_training} summarizes the procedure by detailing the required steps and their sequence. After completing the training, several adaptations in the network's structure are required to exploit the effectiveness of the filter-sharing approach. This post-processing scheme is the topic of the following section.

\begin{algorithm}
\caption{Training a L-layer ALF-Net.}
\label{alg:ae_training}
\begin{algorithmic}[1]
\Require a minibatch of inputs and target ($I,Y$), previous weights $W$, $W_{\text{exp}}$,$W_{\text{enc}}$,$W_{\text{dec}}$, $M$,
regularizion coefficient $\nu$ and learning rates $\eta$ and $\eta_{\text{ae}}$.
\Statex \textbf{Forward propagation:}
\For{$l:=1$ to $L$}
    \State $M_{\text{prune}} \gets \clip(M, t)$ \Comment{Eq.~\ref{eq:clip}}
    \State $W_{\text{code}} \gets \sigma_{\text{ae}}((W \cdot W_{\text{enc}}) \odot M_{\text{clip}})$ \Comment{Eq.~\ref{eq:code}}
    \State $A^{l} \gets \sigma(\sigma(A^{l-1} \ast W_{\text{code}}) \ast W_{\text{exp}})$ \Comment{Eq.~\ref{eq:auto_share_inference}}
    \State $W_{\text{rec}} \gets \sigma_{\text{ae}}(W_{\text{code}} \cdot W_{\text{dec}})$ \Comment{Eq.~\ref{eq:rec}}
\EndFor

\Statex \textbf{Backward propagation:}
\State Compute: $\mathcal{L}_{\text{task}}$ and $\mathcal{L}_{\text{ae}}$ \Comment{Eq.~\ref{eq:task_loss}, Eq.~\ref{eq:ae_loss_used} and Eq.~\ref{eq:ae_loss_used}}
\For{$l:=L$ to $1$}
    \State $g_{W_{\text{exp}}}$ using $\mathcal{L}_{\text{task}}$ \Comment{Vanilla Chain-Rule}
    \State $g_{W} \overset{\text{STE}}\gets{} \pdv{\mathcal{L}_{\text{task}}}{\tilde{A}} \cdot \pdv{\tilde{A}}{W_{\text{code}}}$ using $\mathcal{L}_{\text{task}}$ \Comment{Eq.~\ref{eq:grad_w_orig}}
    \State $g_{W_{\text{enc}}}$ and $g_{W_{\text{dec}}}$ using $\mathcal{L}_{\text{ae}}$\Comment{Vanilla Chain-Rule}
    \State $g_{M} \overset{\text{STE}}\gets{} \pdv{\mathcal{L}_{\text{ae}}}{W_{\text{rec}}} \cdot \pdv{{W_{\text{rec}}}}{W_{\text{code}}} \cdot \pdv{{W_{\text{code}}}}{M_{\text{prune}}}$ using $\mathcal{L}_{\text{ae}}$ \Comment{Eq.~\ref{eq:grad_m}}
\EndFor

\Statex \textbf{Accumulating the gradients: (Momentum/Adam)}
\For{$l:=1$ to $L$}
    \State $W$,$W_{\text{exp}}\gets\texttt{Upd}(g_W, g_W_{\text{exp}},\eta)$ \Comment{Task Objective}
    \State $M^{t+1},W^{t+1}_{\text{enc}},W^{t+1}_{\text{dec}}\gets\texttt{Upd}(g_M, g_W_{\text{enc}}, g_W_{\text{dec}},\eta_{\text{ae}})$
\EndFor

\end{algorithmic}
\end{algorithm}

==> data/misc/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tab/tab_alf_reduction.tex <==
\begin{table}
\centering
\caption{Ops/weights of a Conv layer and an ALF-block.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcc}
    \toprule
    \textbf{KPI\textbackslash Layer}&\textbf{Conv}&\textbf{ALF}\\
    \midrule
    \midrule
    \textbf{\#MACs}& $C_i C_o K^2 H_o W_o$&$\underbrace{2 \cdot C_i C_{\text{code}} K^2 H_o W_o}_{\text{Code layer}} + \underbrace{2 \cdot C_o C_{\text{code}} H_o W_o}_{\text{Expansion layer}}$\\
    \textbf{\#Params}&$C_i C_o K^2$&$\underbrace{C_i C_{\text{code}} K^2}_{\text{Code layer}} + \underbrace{C_{\text{code}} C_o}_{\text{Expansion layer}}$\\
    \midrule
    \textbf{Improvement}&\multicolumn{2}{c}{$\frac{C_i C_o K^2}{C_{\text{code}} (C_i K^2 + C_o)}\rightarrow C_{\text{code,max}}=\lfloor\frac{C_iC_oK^2}{C_iK^2+C_o}\rfloor$}\\
    \bottomrule
    \end{tabular}}
    \vspace{-3mm}
    \label{tab:resources_filter_sharing}
\end{table}

==> tab/tab_ilsvrc_benchmark.tex <==
\begin{table}[!h]
\vspace{-1ex}
\centering
\caption[Benchmarking results on ImageNet.]{Benchmarking results on ImageNet, comparing models and methods with regard to $\mathtt{OPs}$ and $\mathtt{Params}$.}
  \label{tab:benchmarking_ilsvrc_alf}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{llccc}
  \toprule
  \textbf{Method}&\textbf{Policy}&$\mathtt{Params}$&$\mathtt{OPs}$ [$10^6$]&\textbf{Acc [\%]}\\
    \midrule
    \midrule
    SqueezeNet~\cite{squeezenet} & --- & \textbf{1.25M} & 3400 & 57.2~\% \\
    GoogleNet~\cite{googlenet} & --- & 12.75M & 2050 & 66.8\%\\\vspace{2mm}
%    0.5 MobileNet-160~\cite{howard2017mobilenets}  & --- & 1.32M & 152 & 60.2~\%\\
    
    ResNet-18~\cite{resnet} & --- &11.68M & 2330 & \textbf{69.8~\%} \\

    \multicolumn{2}{l}{\textbf{Pruned ResNet-18:} }&&&\\
    \midrule
    LCNN~\cite{lcnn} & Learned  & -- & \textbf{711} & 62.2~\% \\
    FPGM~\cite{geometric_mean_filter} & Hand. & -- & 1356 & 67.8~\% \\
    AMC~\cite{amc} & RL-Agent.&&&67.7~\%\\
    ALF (ours) & Automatic ($t=10^{-4}$) & 4.24M & 1033 & 64.3~\%\\
    \bottomrule
    \end{tabular}}
    \vspace{-1ex}
\end{table}


% \begin{table}[!h]
% \centering
% \caption[Benchmarking results on ImageNet.]{Benchmarking results on ImageNet, comparing models and methods with regard to Normalized energy and latency}
%   \label{tab:benchmarking_ilsvrc_alf}
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{V{.3} V{.1} V{.15} V{.15} V{.1} V{.1}} 
%   \toprule
%   \textbf{Model}&\textbf{Method}&\textbf{Params}&\textbf{MOPS$^{1}$}&\textbf{Acc [\%]}\\
%     \midrule
%     GoogleNet~\cite{qiu2016going} & -  & \textbf{69.83~\%} & 3100 & 6.8\\
%     0.5 MobileNet-160~\cite{howard2017mobilenets}  & - & 60.2~\% & \textbf{152} & 1.32\\
%     SqueezeNet~\cite{iandola2016squeezenet} & -& 57.2~\% & 3400 & ~\textbf{1.25} \\
%     \midrule
%     ResNet-18~\cite{he2016deep} & - & \textbf{69.83~\%}$^{1}$ & 3555 & 11.68\\
%     ResNet-18~\cite{he2016deep} & LCNN~\cite{bagherinezhad2017lcnn}  & 62.2~\% & 711 & - \\
    
%     ResNet-18~\cite{he2016deep} & SFP~\cite{he2018soft} & 67.10~\% & 2031 & - \\
%     \midrule
%     ResNet-18~\cite{he2016deep} & ALF (ours) & 64.33~\% & 1033239 & 4.24\\
%     \bottomrule
%     \end{tabular}}
% \end{table}
